Few-Shot Scene Adaptive Crowd Counting Using Meta-Learning

We consider the problem of few-shot scene adaptive crowd counting. Given a target camera scene, our goal is to adapt a model to this specific scene with only a few labeled images of that scene. The solution to this problem has potential applications in numerous real-world scenarios, where we ideally like to deploy a crowd counting model specially adapted to a target camera. We accomplish this challenge by taking inspiration from the recently introduced learning-to-learn paradigm in the context of few-shot regime. In training, our method learns the model parameters in a way that facilitates the fast adaptation to the target scene. At test time, given a target scene with a small number of labeled data, our method quickly adapts to that scene with a few gradient updates to the learned parameters. Our extensive experimental results show that the proposed approach outperforms other alternatives in few-shot scene adaptive crowd counting. Code is available at https://github.com/maheshkkumar/fscc.

==> algorithm.tex <==
% Algorithm 
\begin{algorithm*}[H]
 \textbf{Input}: Meta-train data $\mathcal{D}_{meta-train}$, meta-test data $\mathcal{D}_{meta-test}$, inner-update learning rate $\alpha$, outer-update learning rate $\beta$,  $K \in \{1, 5\}$ images for training per scene%, $N$ total scenes in $\mathcal{D}_{meta-train}$ %Number of inner tasks $T$ per iteration, episode length of each task $L$, 
 \\
 \textbf{Output}: Learned parameters $\theta$ \\
 Initialize $\theta$ with weights from \textit{pre-trained} model \\
 %Freeze \textit{feature extractor} and train only \textit{density map estimator}  \\
  \tcc{Performing meta-training}
 \While{not done}{
  %\eIf{K = 1}{
  % T = 32
  % }{
  % T = 16
  %}
  Sample $N$ tasks, where $N \in \mathcal{D}_{meta-train}$%, with episode length L = 1 
  \\
  \tcc{Performing inner-update}
  \ForEach{$\mathcal{T}_{i}$ in $N$}{
  	%Sample ($\mathcal{D}_{i}^{train}$, $\mathcal{D}_{i}^{test}$) = $\mathcal{T}_{i}$ \\
  	Sample $K$ images, $D^{train}_{i} = \{x^{(j)}, y^{(j)}\}$ from $\mathcal{T}_{i}$ \\
  	Calculate the gradients $\nabla_{\theta}\mathcal{L}_{\mathcal{T}_{i}}(f_{\theta})$ on $D_{i}^{train}$ based on the loss function defined in $\mathcal{L}_{\mathcal{T}_{i}} $ in Eq.~\ref{eq:inner_update} \\
  	Update the scene-specific parameters $\tilde{\theta_{i}} = \theta - \alpha \nabla_{\theta} \mathcal{L}_{\mathcal{T}_{i}}(f_{\theta})$ based on gradient descent \\ 
  	Sample $K$ images, $D^{test}_{i} = \{x^{(j)}, y^{(j)}\}$ from $\mathcal{T}_{i}$ \\
  	 Compute the objective of $\widehat{\mathcal{L}}_{\mathcal{T}_i}(f_{\tilde{\theta_{i}}})=\sum_{(x^{(j)}, y^{(j)}) \in D_{i}^{test}}\|f_{\tilde{\theta_{i}}}(x^{(j)}) - y^{(j)}\|_{F}^{2}$ \\
  }
  \tcc{Performing outer-update}
  Update $\theta = \theta - \beta \nabla_{\theta} \sum_{i=1}^N \widehat{\mathcal{L}}_{\mathcal{T}_i}(f_{\tilde{\theta_{i}}})$\\ 
 }
 \tcc{Performing meta-testing}
 Adapt to a scene in $\mathcal{D}_{meta-test}$ using the generalizable parameters $\theta$ by performing few gradient updates on $K$ images in $D^{train}_{meta-test}$ and testing on the rest of the images in $D^{test}_{meta-test}$
 \caption{Scene-adaptive Crowd Counting Algorithm}
 \label{alg:meta-learning}
\end{algorithm*}

==> fig_qualitative_images.tex <==
\begin{figure}[!ht]
	\centering
	{\setlength\tabcolsep{1pt}
		\begin{tabular}{ccccc}
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_2_input_v1.png} &
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_2_gt_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_2_ours_v2.png} & \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_2_fine_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_2_pre_v2.png} \\
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_3_input_v1.png} &
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_3_gt_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_3_ours_v2.png} & \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_3_fine_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_3_pre_v2.png} \\
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_4_input_v1.png} &
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_4_gt_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_4_ours_v2.png} & \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_4_fine_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_4_pre_v2.png} \\
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_5_input_v1.png} &
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_5_gt_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_5_ours_v2.png} & \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_5_fine_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/scene_5_pre_v2.png} \\
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/mall_input_v1.png} &
			\includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/mall_gt_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/mall_ours_v2.png} & \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/mall_fine_v2.png} &   \includegraphics[width=3.3cm,height=2.1cm]{qualitative_images/mall_pre_v2.png} \\
			(a) Input Image & (b) Ground-truth & (c) Ours & (d) Baseline fine-tuned & (e) Baseline pre-trained \\
		\end{tabular}
	}
	%\caption{Qualitative results showing the generated density maps from all the models. The first column is the input image, second column is the ground-truth density map, third column shows the map generated by our model, fourth column shows the density map generated by the fine-tuned model, and last column is the output from pre-trained model. The two rows correspond to WorldExpo'10~\cite{zhang2015crosscounting} dataset.}
	\caption{Qualitative results showing the generated density maps for different models. Here we include, (a) input scene-specific crowd image, (b) the corresponding ground-truth (GT), (c) predictions (estimated count) from our proposed approach, (d) predictions from fine-tuned baseline and (e) predictions from pre-trained baseline. The first four rows are the test scenes from WorldExpo'10~\cite{zhang2015crosscounting} and the last row is the test scene from Mall~\cite{loy13_iccvcounting} dataset.} 
	\label{fig:qualitative_images}
\end{figure}



==> fig_sensitivity.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=8.5cm,height=3.0cm]{qualitative_images/sensitivity/Mall_shots_5.png} &   \includegraphics[width=8.5cm,height=3.0cm]{qualitative_images/sensitivity/WorldExpo_scene_4_shots_5.png} \\
		(a) UCSD & (b) WorldExpo Scene 4\\ 
	\end{tabular}
	\caption{Analysis of network sensitivity on the target scene. The labels include, (a) Mall, (b) WorldExpo Scene 4. From the figure, we can infer that the sensitivity or the pertubation is higher for layers in density map estimator (dme) compared to the feature extractor (fe) part of the network.}
	\label{fig:count_sensitivity}
\end{figure*}


==> tab_mall.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{ccccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{1-shot (K=1)}}            & \multicolumn{3}{c}{\textbf{5-shot (K=5)}}            \\
                                  & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               \\ \cline{2-7}
Pre-trained                       & 7.29            & 7.96            & 0.22              & 7.29            & 7.96            & 0.22              \\ 
Fine-tuned                        & 7.11 $\pm$ {\footnotesize 0.09} & 7.80 $\pm$ {\footnotesize 0.08} & 0.21 $\pm$ {\footnotesize 0.003}  & 6.58 $\pm$ {\footnotesize 0.07} & 7.32 $\pm$ {\footnotesize 0.06} & 0.20 $\pm$ {\footnotesize 0.002}  \\ 
\textbf{Ours w/o ROI}                    & 2.52 $\pm$ 0.08 & 3.26 $\pm$ {\footnotesize 0.12} & 0.078 $\pm$ {\footnotesize 0.002} & 2.53 $\pm$ {\footnotesize 0.18} & 3.25 $\pm$ {\footnotesize 0.27} & 0.078 $\pm$ {\footnotesize 0.004} \\ 
\textbf{Ours w/ ROI}                   & \textbf{2.44 $\pm$ {\footnotesize 0.02}} & \textbf{3.12 $\pm$ {\footnotesize 0.03}} & \textbf{0.076 $\pm$ {\footnotesize 0.001}}  & \textbf{2.37 $\pm$ {\footnotesize 0.02}} & \textbf{3.04 $\pm$ {\footnotesize 0.01}} & \textbf{0.073 $\pm$ {\footnotesize 0.001}}  \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\caption{The overall results for adaptation on from WorldExpo'10~\cite{zhang2015crosscounting} to Mall~\cite{change2013semicounting} dataset with $K=1$ and $K=5$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours w/ ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result.}
\label{tab:worldexpo_mall}
\end{table*}


==> tab_mall_v2.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{ccccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{1-shot (K=1)}}            & \multicolumn{3}{c}{\textbf{5-shot (K=5)}}            \\
                                  & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               \\ \cline{2-7}
Baseline Pre-trained                       & 7.29            & 7.96            & 0.22              & 7.29            & 7.96            & 0.22              \\ 
Baseline Fine-tuned                        & 7.11 $\pm$ {\footnotesize 0.09} & 7.80 $\pm$ {\footnotesize 0.08} & 0.21 $\pm$ {\footnotesize 0.003}  & 6.58 $\pm$ {\footnotesize 0.07} & 7.32 $\pm$ {\footnotesize 0.06} & 0.20 $\pm$ {\footnotesize 0.002}  \\ 
\textbf{Reptile}~\cite{nichol2018first}             & 2.55 $\pm$ {\footnotesize 0.07}           & 3.26 $\pm$ {\footnotesize 0.09}  & 0.07 $\pm$ {\footnotesize 0.001}           & 2.49 $\pm$ {\footnotesize 0.23}           & 3.20 $\pm$ {\footnotesize 0.29}          & 0.07 $\pm$ {\footnotesize 0.006}   \\
 \textbf{Meta pre-trained (Ours)} & 7.01 & 7.69 & 0.230 & 7.01 & 7.69 & 0.230 \\
\textbf{Meta fine-tuned (Ours)}                    & 2.52 $\pm$ 0.08 & 3.26 $\pm$ {\footnotesize 0.12} & 0.078 $\pm$ {\footnotesize 0.002} & 2.53 $\pm$ {\footnotesize 0.18} & 3.25 $\pm$ {\footnotesize 0.27} & 0.078 $\pm$ {\footnotesize 0.004} \\ 
\textbf{Meta fine-tuned (Ours w/ ROI)}                   & \textbf{2.44 $\pm$ {\footnotesize 0.02}} & \textbf{3.12 $\pm$ {\footnotesize 0.03}} & \textbf{0.076 $\pm$ {\footnotesize 0.001}}  & \textbf{2.37 $\pm$ {\footnotesize 0.02}} & \textbf{3.04 $\pm$ {\footnotesize 0.01}} & \textbf{0.073 $\pm$ {\footnotesize 0.001}}  \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\caption{{\color{blue} [[To-do: Update the caption]] }The overall results for adaptation on from WorldExpo'10~\cite{zhang2015crosscounting} to Mall~\cite{change2013semicounting} dataset with $K=1$ and $K=5$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours w/ ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result.}
\label{tab:worldexpo_mall}
\end{table*}


==> tab_ucsd.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{ccccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{1-shot (K=1)}}            & \multicolumn{3}{c}{\textbf{5-shot (K=5)}}            \\
                                  & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               \\ \cline{2-7}
Pre-trained                       & 17.07            & 18.13            & 0.63             & 17.07            & 18.13            & 0.70             \\ 
Fine-tuned                        & 16.41 $\pm$ {\footnotesize 0.24} & 17.50 $\pm$ {\footnotesize 0.23} & 0.60 $\pm$ {\footnotesize 0.010} & 14.33 $\pm$ {\footnotesize 0.16} & 15.55 $\pm$ {\footnotesize 0.15} & 0.54 $\pm$ {\footnotesize 0.006} \\ 
\textbf{Ours w/o ROI }                   & 4.32 $\pm$ {\footnotesize 0.74}  & 5.57 $\pm$ {\footnotesize 0.98}  & 0.15 $\pm$ {\footnotesize 0.022}  & 3.82 $\pm$ {\footnotesize 0.39}  & 4.87 $\pm$ {\footnotesize 0.58}  & 0.14 $\pm$ {\footnotesize 0.012} \\
\textbf{Ours w/ ROI}                   & \textbf{3.08 $\pm$ {\footnotesize 0.13}}  & \textbf{4.16 $\pm$ {\footnotesize 0.23}}  & \textbf{0.12 $\pm$ {\footnotesize 0.005}} & \textbf{3.41 $\pm$ {\footnotesize 0.26}}  & \textbf{4.22 $\pm$ {\footnotesize 0.36}}  & \textbf{0.12 $\pm$ {\footnotesize 0.007}}  \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\caption{The overall results for adaptation on from WorldExpo'10~\cite{zhang2015crosscounting} to UCSD~\cite{chan2008privacycounting} dataset with $K=1$ and $K=5$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours w/ ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result.}
\label{tab:worldexpo_ucsd}
\end{table*}


==> tab_ucsd_v2.tex <==
\begin{table*}[!ht]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{ccccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{1-shot (K=1)}}            & \multicolumn{3}{c}{\textbf{5-shot (K=5)}}            \\
                                  & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               & \multicolumn{1}{c}{MAE}             & \multicolumn{1}{c}{RMSE}             & \multicolumn{1}{c}{MDE}               \\ \cline{2-7}
Baseline Pre-trained                       & 17.07            & 18.13            & 0.63             & 17.07            & 18.13            & 0.70             \\ 
Baseline Fine-tuned                        & 16.41 $\pm$ {\footnotesize 0.24} & 17.50 $\pm$ {\footnotesize 0.23} & 0.60 $\pm$ {\footnotesize 0.010} & 14.33 $\pm$ {\footnotesize 0.16} & 15.55 $\pm$ {\footnotesize 0.15} & 0.54 $\pm$ {\footnotesize 0.006} \\ 
\textbf{Reptile}~\cite{nichol2018first}             & 5.64 $\pm$ {\footnotesize 2.05}           & 6.85 $\pm$ {\footnotesize 2.06}  & 0.20 $\pm$ {\footnotesize 0.075}           & 4.48 $\pm$ {\footnotesize 0.88}           & 5.62 $\pm$ {\footnotesize 0.99}          & 0.166 $\pm$ {\footnotesize 0.033}   \\
\textbf{Meta pre-trained (Ours)}             & 16.45 & 16.7 & 0.627 & 16.45 & 16.7 & 0.627 \\
\textbf{Meta fine-tuned (Ours)}                   & 4.32 $\pm$ {\footnotesize 0.74}  & 5.57 $\pm$ {\footnotesize 0.98}  & 0.15 $\pm$ {\footnotesize 0.022}  & 3.82 $\pm$ {\footnotesize 0.39}  & 4.87 $\pm$ {\footnotesize 0.58}  & 0.14 $\pm$ {\footnotesize 0.012} \\
\textbf{Meta fine-tuned (Ours w/ ROI)}                   & \textbf{3.08 $\pm$ {\footnotesize 0.13}}  & \textbf{4.16 $\pm$ {\footnotesize 0.23}}  & \textbf{0.12 $\pm$ {\footnotesize 0.005}} & \textbf{3.41 $\pm$ {\footnotesize 0.26}}  & \textbf{4.22 $\pm$ {\footnotesize 0.36}}  & \textbf{0.12 $\pm$ {\footnotesize 0.007}}  \\ \Xhline{2\arrayrulewidth}
\end{tabular}
\caption{{\color{blue} [[To-do: Update the caption]] }The overall results for adaptation on from WorldExpo'10~\cite{zhang2015crosscounting} to UCSD~\cite{chan2008privacycounting} dataset with $K=1$ and $K=5$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours w/ ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result.}
\label{tab:worldexpo_ucsd}
\end{table*}


==> tab_worldexpo.tex <==
% K=1 and K=5

\begin{table*}[!ht]
  \centering
  \small
  \resizebox{0.9\textwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{cccccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Target}} & \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{1-shot (K=1)}}                                         & \multicolumn{3}{c}{\textbf{5-shot (K=5)}}                                         \\ 
                                 &                                   & \multicolumn{1}{c}{MAE}                       & \multicolumn{1}{c}{RMSE}                       & \multicolumn{1}{c}{MDE}                        & \multicolumn{1}{c}{MAE}                       & \multicolumn{1}{c}{RMSE}                       & \multicolumn{1}{c}{MDE}                        \\ \cline{2-8} 
\multirow{4}{*}{Scene 1}         & Pre-trained                       & 5.55                      & 6.31                      & 0.70                       & 5.55                      & 6.31                      & 0.70                       \\ 
                                 & Fine-tuned                        & 5.45 $\pm$ {\footnotesize 0.03}           & 6.23 $\pm$ {\footnotesize 0.03}           & 0.68 $\pm$ {\footnotesize 0.004}           & 5.06 $\pm$ {\footnotesize 0.11}           & 5.88 $\pm$ {\footnotesize 0.10}           & 0.63 $\pm$ {\footnotesize 0.005}           \\ 
                                 & \textbf{Ours w/o ROI}             & 3.47 $\pm$ {\footnotesize 0.01}           & \textbf{4.19 $\pm$ {\footnotesize 0.01}}  & 0.50 $\pm$ {\footnotesize 0.007}           & 3.42 $\pm$ {\footnotesize 0.03}           & 4.81 $\pm$ {\footnotesize 0.007}          & \textbf{0.29 $\pm$ {\footnotesize 0.004}}   \\ 
                                 & \textbf{Ours w/ ROI}            & \textbf{3.19 $\pm$ {\footnotesize 0.03}}  & 4.30 $\pm$ {\footnotesize 0.07}           & \textbf{0.38 $\pm$ {\footnotesize 0.03}}   & \textbf{3.05 $\pm$ {\footnotesize 0.06}}  & \textbf{4.19 $\pm$ {\footnotesize 0.15}}  & 0.31 $\pm$ {\footnotesize 0.08}            \\ \hline
\multirow{4}{*}{Scene 2}         & Pre-trained                       & 24.07                     & 34.29                     & 0.17                       & 24.07                     & 34.29                     & 0.17                       \\ 
                                 & Fine-tuned                        & 22.74 $\pm$ {\footnotesize 0.47}          & 32.92 $\pm$ {\footnotesize 0.66}          & 0.15 $\pm$ {\footnotesize 0.003}           & 20.84 $\pm$ {\footnotesize 1.03}          & 30.49 $\pm$ {\footnotesize 1.37}          & 0.156 $\pm$ {\footnotesize 0.001}          \\
                                 & \textbf{Ours w/o ROI}             & 12.05 $\pm$ {\footnotesize 0.74}          & 16.62 $\pm$ {\footnotesize 1.10}          & 0.11 $\pm$ {\footnotesize 0.007}           & 11.41 $\pm$ {\footnotesize 0.54}          & 15.35 $\pm$ {\footnotesize 0.51}          & 0.11 $\pm$ {\footnotesize 0.015}           \\
                                 & \textbf{Ours w/ ROI}            & \textbf{11.17 $\pm$ {\footnotesize 1.01}} & \textbf{15.50 $\pm$ {\footnotesize 1.18}} & \textbf{0.11 $\pm$ {\footnotesize 0.012}}  & \textbf{10.73 $\pm$ {\footnotesize 0.36}} & \textbf{14.95 $\pm$ {\footnotesize 0.60}} & \textbf{0.10 $\pm$ {\footnotesize 0.003}}  \\ \hline
\multirow{4}{*}{Scene 3}         & Pre-trained                       & 35.54                     & 40.78                     & 0.40                       & 35.54                     & 40.78                     & 0.40                       \\
                                 & Fine-tuned                        & 33.89 $\pm$ {\footnotesize 0.26}          & 39.33 $\pm$ {\footnotesize 0.25}          & 0.38 $\pm$ {\footnotesize 0.03}            & 31.05 $\pm$ {\footnotesize 0.41}          & 36.70 $\pm$ {\footnotesize 0.43}          & 0.34 $\pm$ {\footnotesize 0.004}           \\ 
                                 & \textbf{Ours w/o ROI}             & 8.15 $\pm$ {\footnotesize 0.17}           & 11.04 $\pm$ {\footnotesize 0.42}          & \textbf{0.09 $\pm$ {\footnotesize 0.04}}  & 8.31 $\pm$ {\footnotesize 0.54}           & \textbf{10.75 $\pm$ {\footnotesize 0.54}} & 0.10 $\pm$ {\footnotesize 0.009}          \\
                                 & \textbf{Ours w/ ROI}            & \textbf{8.07 $\pm$ {\footnotesize 0.23}}  & \textbf{10.92 $\pm$ {\footnotesize 0.21}} & 0.10 $\pm$ {\footnotesize 0.007}           & \textbf{8.18 $\pm$ {\footnotesize 0.24}}  & 10.96 $\pm$ {\footnotesize 0.31}          & \textbf{0.09 $\pm$ {\footnotesize 0.002}} \\ \hline
\multirow{4}{*}{Scene 4}         & Pre-trained                       & 23.95                     & 28.57                     & 0.19                       & 23.95                     & 28.57                     & 0.19                       \\ 
                                 & Fine-tuned                        & 15.69 $\pm$ {\footnotesize 0.28}          & 18.96 $\pm$ {\footnotesize 0.27}          & 0.14 $\pm$ {\footnotesize 0.003}           & 16.67 $\pm$ {\footnotesize 0.10}          & 19.70 $\pm$ {\footnotesize 0.16}          & 0.15 $\pm$ {\footnotesize 0.002}           \\ 
                                 & \textbf{Ours w/o ROI}             & 9.74 $\pm$ {\footnotesize 0.09}          & 11.9 $\pm$ {\footnotesize 0.12}          & 0.084 $\pm$ {\footnotesize 0.001}           & 11.21 $\pm$ {\footnotesize 0.47}          & 16.1 $\pm$ {\footnotesize 0.45}          & 0.118 $\pm$ {\footnotesize 0.004}           \\ 
                                 & \textbf{Ours w/ ROI}            & \textbf{9.39 $\pm$ {\footnotesize 0.26}} & \textbf{11.78 $\pm$ {\footnotesize 0.34}} & \textbf{0.07 $\pm$ {\footnotesize 0.02}}  & \textbf{9.41 $\pm$ {\footnotesize 0.21}} & \textbf{11.91 $\pm$ {\footnotesize 0.17}} & \textbf{0.08 $\pm$ {\footnotesize 0.002}}   \\ \hline
\multirow{4}{*}{Scene 5}         & Pre-trained                       & 10.70                     & 13.0                      & 0.67                       & 10.70                     & 13.0                      & 0.67                       \\  
                                 & Fine-tuned                        & 8.9 $\pm$ {\footnotesize 0.05}            & 11.7 $\pm$ {\footnotesize 0.04}           & 0.50 $\pm$ {\footnotesize 0.03}            & 7.79 $\pm$ {\footnotesize 0.35}           & 10.57 $\pm$ {\footnotesize 0.66}          & 0.44 $\pm$ {\footnotesize 0.015}           \\  
                                 & \textbf{Ours w/o ROI}             & 4.09 $\pm$ {\footnotesize 0.01}           & 7.36 $\pm$ {\footnotesize 0.01}           & 0.196 $\pm$ {\footnotesize 0.001}           & 4.28 $\pm$ {\footnotesize 0.14}           & 7.68 $\pm$ {\footnotesize 0.60}           & 0.20 $\pm$ {\footnotesize 0.001}           \\  
                                 & \textbf{Ours w/ ROI}            & \textbf{3.82 $\pm$ {\footnotesize 0.05}}  & \textbf{6.91 $\pm$ {\footnotesize 0.11}}  & \textbf{0.192 $\pm$ {\footnotesize 0.001}} & \textbf{3.91 $\pm$ {\footnotesize 0.26}}  & \textbf{7.18 $\pm$ {\footnotesize 0.85}}  & \textbf{0.18 $\pm$ {\footnotesize 0.001}} \\ \hline
\multirow{4}{*}{\textbf{Average}}   & Pre-trained                       & 19.96                     & 24.59                      & 0.42                       & 19.96                     & 24.59                      & 0.42                       \\  
                                 & Fine-tuned                        & 17.33 & 21.82            & 0.37 & 16.28           & 20.66            & 0.34                         \\ 
                                 & \textbf{Ours w/o ROI}             & 7.5                 & 10.22                 & 0.197                  & 7.7                 & 10.93                 & 0.165                  \\  
                                 & \textbf{Ours w/ ROI}            & \textbf{7.12}                      & \textbf{9.88}                         & \textbf{0.172 }                          & \textbf{7.05                         } & \textbf{9.83}                           & \textbf{0.155} \\ \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{The overall results for adaptation on WorldExpo'10~\cite{zhang2015crosscounting} test set with $K = 1$ and $K = 5$ train images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours w/ ROI''} and \textit{``Ours w/o ROI''}. We compare the results across 5 test scenes and the last two rows represent the average score for our models. The results in bold represent the overall best result. }
\label{tab:worldexpo}
\end{table*}


% K=1
%\begin{table}[]
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\textbf{Target}}               & \multirow{2}{*}{\textbf{Methods}}       & \multicolumn{3}{c|}{\textbf{5-shot (K=5)}}                                                                                           \\
 %                                              &                                         & \multicolumn{1}{c}{MAE}                                        & \multicolumn{1}{c}{MSE}                                        & \multicolumn{1}{c|}{MDE}                                         \\ \hline
%\multirow{4}{*}{Scene 1}         & Pre-trained                       & 5.55                      & 6.31                      & 0.70                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 5.45 $\pm$ 0.03           & 6.23 $\pm$ 0.03           & 0.68 $\pm$ 0.004           \\ \cline{2-5} 
 %                                & \textbf{Ours w/o ROI}             & 3.47 $\pm$ 0.01           & \textbf{4.19 $\pm$ 0.01}  & 0.50 $\pm$ 0.007           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{3.19 $\pm$ 0.03}  & 4.30 $\pm$ 0.07           & \textbf{0.38 $\pm$ 0.03}   \\ \hline
%\multirow{4}{*}{Scene 2}         & Pre-trained                       & 24.07                     & 34.29                     & 0.17                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 22.74 $\pm$ 0.47          & 32.92 $\pm$ 0.66          & 0.15 $\pm$ 0.003           \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 12.05 $\pm$ 0.74          & 16.62 $\pm$ 1.10          & 0.11 $\pm$ 0.007           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{11.17 $\pm$ 1.01} & \textbf{15.50 $\pm$ 1.18} & \textbf{0.11 $\pm$ 0.012}  \\ \hline
%\multirow{4}{*}{Scene 3}         & Pre-trained                       & 35.54                     & 40.78                     & 0.40                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 33.89 $\pm$ 0.26          & 39.33 $\pm$ 0.25          & 0.38 $\pm$ 0.03            \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 8.15 $\pm$ 0.17           & 11.04 $\pm$ 0.42          & 0.098 $\pm$ 0.04           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{8.07 $\pm$ 0.23}  & \textbf{10.92 $\pm$ 0.21} & \textbf{0.10 $\pm$ 0.007}  \\ \hline
%\multirow{4}{*}{Scene 4}         & Pre-trained                       & 23.95                     & 28.57                     & 0.19                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 15.69 $\pm$ 0.28          & 18.96 $\pm$ 0.27          & 0.14 $\pm$ 0.003           \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 16.64 $\pm$ 0.24          & 20.35 $\pm$ 0.25          & 0.14 $\pm$ 0.002           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{15.55 $\pm$ 0.09} & \textbf{18.94 $\pm$ 0.12} & \textbf{0.13 $\pm$ 0.001}  \\ \hline
%\multirow{4}{*}{Scene 5}         & Pre-trained                       & 10.70                     & 13.0                      & 0.67                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 8.9 $\pm$ 0.05            & 11.7 $\pm$ 0.04           & 0.50 $\pm$ 0.03            \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 4.09 $\pm$ 0.01           & 7.36 $\pm$ 0.01           & 0.196 $\pm$ 0.01           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{3.82 $\pm$ 0.05}  & \textbf{6.91 $\pm$ 0.11}  & \textbf{0.192 $\pm$ 0.001} \\ \hline
%\end{tabular}
%\caption{The overall results for adaptation on WorldExpo test set with $K = 1$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours with ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result achieved by our model.}
%\label{tab:worldexpo_k1}
%\end{table}

% K = 5
%\begin{table}[]
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\textbf{Target}}               & \multirow{2}{*}{\textbf{Methods}}       & \multicolumn{3}{c|}{\textbf{5-shot (K=5)}}                                                                                           \\
%                                               &                                         & \multicolumn{1}{c}{MAE}                                        & \multicolumn{1}{c}{MSE}                                        & \multicolumn{1}{c|}{MDE}                                         \\ \hline
%\multirow{4}{*}{Scene 1}                       & Pre-trained                             & 5.55                                       & 6.31                                       & 0.70                                        \\ \cline{2-5} 
%                                               & Fine-tuned                              & 5.06 $\pm$ 0.11                            & 5.88 $\pm$ 0.10                            & 0.63 $\pm$ 0.005                            \\ \cline{2-5} 
%                                               & \textbf{Ours w/o ROI}  & 3.42 $\pm$ 0.03                            & 4.81 $\pm$ 0.007                           & \textbf{0.29 $\pm$ 0.04}   \\ \cline{2-5} 
%                                               & \textbf{Ours with ROI} & \textbf{3.05 $\pm$ 0.06}  & \textbf{4.19 $\pm$ 0.15}  & 0.31 $\pm$ 0.08                             \\ \hline
%\multirow{4}{*}{Scene 2}                       & Pre-trained                             & 24.07                                      & 34.29                                      & 0.17                                        \\ \cline{2-5} 
%                                               & Fine-tuned                              & 20.84 $\pm$ 1.03                           & 30.49 $\pm$ 1.37                           & 0.156 $\pm$ 0.001                           \\ \cline{2-5} 
%                                               & \textbf{Ours w/o ROI}  & 11.41 $\pm$ 0.54                           & 15.35 $\pm$ 0.51                           & 0.11 $\pm$ 0.015                            \\ \cline{2-5} 
%                                               & \textbf{Ours with ROI} & \textbf{10.73 $\pm$ 0.36} & \textbf{14.95 $\pm$ 0.60} & \textbf{0.10 $\pm$ 0.003}  \\ \hline
%\multirow{4}{*}{Scene 3}                       & Pre-trained                             & 35.54                                      & 40.78                                      & 0.40                                        \\ \cline{2-5} 
%                                               & Fine-tuned                              & 31.05 $\pm$ 0.41                           & 36.70 $\pm$ 0.43                           & 0.34 $\pm$ 0.004                            \\ \cline{2-5} 
%                                               & \textbf{Ours w/o ROI}  & 8.31 $\pm$ 0.54                            & \textbf{10.75 $\pm$ 0.54} & 0.109 $\pm$ 0.009                           \\ \cline{2-5} 
%                                               & \textbf{Ours with ROI} & \textbf{8.18 $\pm$ 0.24}  & 10.96 $\pm$ 0.31                           & \textbf{0.098 $\pm$ 0.002} \\ \hline
%\multicolumn{1}{|l|}{\multirow{4}{*}{Scene 4}} & Pre-trained                             & 23.95                                      & 28.57                                      & 0.19                                        \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & Fine-tuned                              & 16.67 $\pm$ 0.10                           & 19.70 $\pm$ 0.16                           & 0.15 $\pm$ 0.002                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours w/o ROI}  & 16.92 $\pm$ 0.52                           & 20.07 $\pm$ 0.49                           & 0.15 $\pm$ 0.004                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours with ROI} & \textbf{11.65 $\pm$ 0.59} & \textbf{15.26 $\pm$ 0.94} & \textbf{0.09 $\pm$ 0.05}   \\ \hline
%\multicolumn{1}{|l|}{\multirow{4}{*}{Scene 5}} & Pre-trained                             & 10.70                                      & 13.0                                       & 0.67                                        \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & Fine-tuned                              & 7.79 $\pm$ 0.35                            & 10.57 $\pm$ 0.66                           & 0.44 $\pm$ 0.015                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours w/o ROI}  & 4.28 $\pm$ 0.14                            & 7.68 $\pm$ 0.60                            & 0.20 $\pm$ 0.001                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours with ROI} & \textbf{3.91 $\pm$ 0.26}  & \textbf{7.18 $\pm$ 0.85}  & \textbf{0.187 $\pm$ 0.001} \\ \cline{1-5} 
%\end{tabular}
%\caption{The overall results for adaptation on WorldExpo test set with $K = 5$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours with ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result achieved by our model.}
%\label{tab:worldexpo_k5}
%\end{table}

%\begin{table}[]
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Methods}    & \textbf{Scene 1} & \textbf{Scene 2} & \textbf{Scene 3} & \textbf{Scene 4} & \textbf{Scene 5} & \textbf{Average} \\ \hline
%Chen et al.         & \textbf{2.1}     & 55.9             & 9.6              & 11.3             & 3.4              & 16.5             \\ \hline
%Zhang et al.        & 9.8              & 14.1             & 14.3             & 22.2             & 3.7              & 12.9             \\ \hline
%MCNN                & 3.4              & 20.6             & 12.9             & 13.0             & 8.1              & 11.6             \\ \hline
%Shang et al.        & 7.8              & 15.4             & 14.9             & 11.8             & 5.8              & 11.7             \\ \hline
%Switching-CNN       & 4.4              & 15.7             & 10.0             & 11.0             & 5.9              & 9.4              \\ \hline
%CP-CNN              & 2.9              & 14.7             & 10.5             & 10.4             & 5.8              & 8.86             \\ \hline
%CSRNet              & 2.9              & 11.5             & 8.6              & 16.6             & 3.4              & 8.6              \\ \hline
%SANet               & 2.6              & 13.2             & 9.0              & 13.3             & \textbf{3.0}     & 8.2              \\ \hline
%PACNN               & 2.3              & 12.5             & 9.1              & \textbf{11.2}    & 3.8              & 7.8              \\ \hline
%\textbf{Ours (K=1)} & 3.1              & 11.1             & \textbf{8.0}     & 15.5             & 3.8              & 8.3              \\ \hline
%\textbf{Ours (K=5)} & 3.0              & \textbf{10.7}    & 8.1              & 11.6             & 3.9              & \textbf{7.4}     \\ \hline
%\end{tabular}
%\caption{Comparison of our approach with previous approaches in Crowd Counting based on the average scores of WorldExpo test set. <\textbf{To-Do}: References>}
%\end{table}


==> tab_worldexpo_v2.tex <==
% K=1 and K=5

\begin{table*}[!ht]
  \centering
  \small
  \resizebox{0.9\textwidth}{!}{%
\def\arraystretch{1.1}
\begin{tabular}{cccccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\textbf{Target}} & \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{1-shot (K=1)}}                                         & \multicolumn{3}{c}{\textbf{5-shot (K=5)}}                                         \\ 
                                 &                                   & \multicolumn{1}{c}{MAE}                       & \multicolumn{1}{c}{RMSE}                       & \multicolumn{1}{c}{MDE}                        & \multicolumn{1}{c}{MAE}                       & \multicolumn{1}{c}{RMSE}                       & \multicolumn{1}{c}{MDE}                        \\ \cline{1-8} 
\multirow{4}{*}{Scene 1}         
& Baseline Pre-trained                       & 5.55                      & 6.31                      & 0.70                       & 5.55                      & 6.31                      & 0.70                       \\ 
& Baseline Fine-tuned                        & 5.45 $\pm$ {\footnotesize 0.03}           & 6.23 $\pm$ {\footnotesize 0.03}           & 0.68 $\pm$ {\footnotesize 0.004}           & 5.06 $\pm$ {\footnotesize 0.11}           & 5.88 $\pm$ {\footnotesize 0.10}           & 0.63 $\pm$ {\footnotesize 0.005}           \\ 
& \textbf{Reptile} ~\cite{nichol2018first}            & 4.99 $\pm$ {\footnotesize 0.46}           & 7.08 $\pm$ {\footnotesize 1.09}  & 0.47 $\pm$ {\footnotesize 0.123}           & 3.38 $\pm$ {\footnotesize 0.59}           & 4.38 $\pm$ {\footnotesize 0.63}          & 0.36 $\pm$ {\footnotesize 0.112}   \\ %\cdashline{2-8}
& \textbf{Meta pre-trained (Ours)}             & 4.63           & 5.5 & 0.529 &  4.63           & 5.5 & 0.529 \\
                                 & \textbf{Meta fine-tuned (Ours)}             & 3.47 $\pm$ {\footnotesize 0.01}           & \textbf{4.19 $\pm$ {\footnotesize 0.01}}  & 0.50 $\pm$ {\footnotesize 0.007}           & 3.42 $\pm$ {\footnotesize 0.03}           & 4.81 $\pm$ {\footnotesize 0.007}          & \textbf{0.29 $\pm$ {\footnotesize 0.004}}   \\ 
                                 & \textbf{Meta fine-tuned (Ours w/ ROI)}            & \textbf{3.19 $\pm$ {\footnotesize 0.03}}  & 4.30 $\pm$ {\footnotesize 0.07}           & \textbf{0.38 $\pm$ {\footnotesize 0.03}}   & \textbf{3.05 $\pm$ {\footnotesize 0.06}}  & \textbf{4.19 $\pm$ {\footnotesize 0.15}}  & 0.31 $\pm$ {\footnotesize 0.08}            \\ \hline
\multirow{4}{*}{Scene 2}          
& Baseline Pre-trained                       & 24.07                     & 34.29                     & 0.17                       & 24.07                     & 34.29                     & 0.17                       \\ 
& Baseline Fine-tuned                        & 22.74 $\pm$ {\footnotesize 0.47}          & 32.92 $\pm$ {\footnotesize 0.66}          & 0.15 $\pm$ {\footnotesize 0.003}           & 20.84 $\pm$ {\footnotesize 1.03}          & 30.49 $\pm$ {\footnotesize 1.37}          & 0.156 $\pm$ {\footnotesize 0.001}          \\
& \textbf{Reptile}~\cite{nichol2018first}             & 21.51 $\pm$ {\footnotesize 0.45}           & 25.85 $\pm$ {\footnotesize 0.48}  & 0.30 $\pm$ {\footnotesize 0.062}           & 14.52 $\pm$ {\footnotesize 3.11}           & 20.46 $\pm$ {\footnotesize 4.29}          & 0.14 $\pm$ {\footnotesize 0.049}   \\ %\cline{2-8}
& \textbf{Meta pre-trained (Ours)}             & 21.65 & 30.51 & 0.185 & 21.65 & 30.51 & 0.185 \\
& \textbf{Meta fine-tuned(Ours)}             & 12.05 $\pm$ {\footnotesize 0.74}          & 16.62 $\pm$ {\footnotesize 1.10}          & 0.11 $\pm$ {\footnotesize 0.007}           & 11.41 $\pm$ {\footnotesize 0.54}          & 15.35 $\pm$ {\footnotesize 0.51}          & 0.11 $\pm$ {\footnotesize 0.015}           \\
& \textbf{Meta fine-tuned (Ours w/ ROI)}            & \textbf{11.17 $\pm$ {\footnotesize 1.01}} & \textbf{15.50 $\pm$ {\footnotesize 1.18}} & \textbf{0.11 $\pm$ {\footnotesize 0.012}}  & \textbf{10.73 $\pm$ {\footnotesize 0.36}} & \textbf{14.95 $\pm$ {\footnotesize 0.60}} & \textbf{0.10 $\pm$ {\footnotesize 0.003}}  \\ \hline
\multirow{4}{*}{Scene 3}         
& Baseline Pre-trained                       & 35.54                     & 40.78                     & 0.40                       & 35.54                     & 40.78                     & 0.40                       \\
& Baseline Fine-tuned                        & 33.89 $\pm$ {\footnotesize 0.26}          & 39.33 $\pm$ {\footnotesize 0.25}          & 0.38 $\pm$ {\footnotesize 0.03}            & 31.05 $\pm$ {\footnotesize 0.41}          & 36.70 $\pm$ {\footnotesize 0.43}          & 0.34 $\pm$ {\footnotesize 0.004}           \\ 
& \textbf{Reptile}~\cite{nichol2018first}             & 14.14 $\pm$ {\footnotesize 1.68}           & 18.04 $\pm$ {\footnotesize 1.71}  & 0.156 $\pm$ {\footnotesize 0.015}           & 9.37 $\pm$ {\footnotesize 1.30}           & 12.04 $\pm$ {\footnotesize 1.27}          & 0.123 $\pm$ {\footnotesize 0.026}   \\ %\cline{2-8}
& \textbf{Meta pre-trained (Ours)}             & 36.18 & 42.32 & 0.402 & 36.18 & 42.32 & 0.402 \\
& \textbf{Meta fine-tuned (Ours)}             & 8.15 $\pm$ {\footnotesize 0.17}           & 11.04 $\pm$ {\footnotesize 0.42}          & \textbf{0.09 $\pm$ {\footnotesize 0.04}}  & 8.31 $\pm$ {\footnotesize 0.54}           & \textbf{10.75 $\pm$ {\footnotesize 0.54}} & 0.10 $\pm$ {\footnotesize 0.009}          \\
& \textbf{Meta fine-tuned (Ours w/ ROI)}            & \textbf{8.07 $\pm$ {\footnotesize 0.23}}  & \textbf{10.92 $\pm$ {\footnotesize 0.21}} & 0.10 $\pm$ {\footnotesize 0.007}           & \textbf{8.18 $\pm$ {\footnotesize 0.24}}  & 10.96 $\pm$ {\footnotesize 0.31}          & \textbf{0.09 $\pm$ {\footnotesize 0.002}} \\ \hline
\multirow{4}{*}{Scene 4}         
& Baseline Pre-trained                       & 23.95                     & 28.57                     & 0.19                       & 23.95                     & 28.57                     & 0.19                       \\ 
& Baseline Fine-tuned                        & 15.69 $\pm$ {\footnotesize 0.28}          & 18.96 $\pm$ {\footnotesize 0.27}          & 0.14 $\pm$ {\footnotesize 0.003}           & 16.67 $\pm$ {\footnotesize 0.10}          & 19.70 $\pm$ {\footnotesize 0.16}          & 0.15 $\pm$ {\footnotesize 0.002}           \\ 
& \textbf{Reptile}~\cite{nichol2018first}             & 12.09 $\pm$ {\footnotesize 1.28}           & 14.64 $\pm$ {\footnotesize 1.09}  & 0.106 $\pm$ {\footnotesize 0.017}           & 9.64 $\pm$ {\footnotesize 1.22}           & 12.11 $\pm$ {\footnotesize 1.34}          & 0.082 $\pm$ {\footnotesize 0.011}   \\ %\cline{2-8}
& \textbf{Meta pre-trained (Ours)}             & 22.44 & 28.25 & 0.183 & 22.44 & 28.25 & 0.183 \\
& \textbf{Meta fine-tuned (Ours)}             & 9.74 $\pm$ {\footnotesize 0.09}          & 11.9 $\pm$ {\footnotesize 0.12}          & 0.084 $\pm$ {\footnotesize 0.001}           & 11.21 $\pm$ {\footnotesize 0.47}          & 16.1 $\pm$ {\footnotesize 0.45}          & 0.118 $\pm$ {\footnotesize 0.004}           \\ 
& \textbf{Meta fine-tuned (Ours w/ ROI)}            & \textbf{9.39 $\pm$ {\footnotesize 0.26}} & \textbf{11.78 $\pm$ {\footnotesize 0.34}} & \textbf{0.07 $\pm$ {\footnotesize 0.02}}  & \textbf{9.41 $\pm$ {\footnotesize 0.21}} & \textbf{11.91 $\pm$ {\footnotesize 0.17}} & \textbf{0.08 $\pm$ {\footnotesize 0.002}}   \\ \hline
\multirow{4}{*}{Scene 5}         
& Baseline Pre-trained                       & 10.70                     & 13.0                      & 0.67                       & 10.70                     & 13.0                      & 0.67                       \\  
 & Baseline Fine-tuned                        & 8.9 $\pm$ {\footnotesize 0.05}            & 11.7 $\pm$ {\footnotesize 0.04}           & 0.50 $\pm$ {\footnotesize 0.03}            & 7.79 $\pm$ {\footnotesize 0.35}           & 10.57 $\pm$ {\footnotesize 0.66}          & 0.44 $\pm$ {\footnotesize 0.015}           \\ 
& \textbf{Reptile}~\cite{nichol2018first}             & 5.42 $\pm$ {\footnotesize 0.32}           & 9.75 $\pm$ {\footnotesize 0.34}  & 0.27 $\pm$ {\footnotesize 0.081}           & 4.10 $\pm$ {\footnotesize 0.66}           & 7.57 $\pm$ {\footnotesize 1.20}          & 0.204 $\pm$ {\footnotesize 0.058}   \\ %\cline{2-8}
& \textbf{Meta pre-trained (Ours)}             & 9.78 & 12.26 & 0.605 & 9.78 & 12.26 & 0.605\\
& \textbf{Meta fine-tuned (Ours)}             & 4.09 $\pm$ {\footnotesize 0.01}           & 7.36 $\pm$ {\footnotesize 0.01}           & 0.196 $\pm$ {\footnotesize 0.001}           & 4.28 $\pm$ {\footnotesize 0.14}           & 7.68 $\pm$ {\footnotesize 0.60}           & 0.20 $\pm$ {\footnotesize 0.001}           \\  
& \textbf{Meta fine-tuned (Ours w/ ROI)}            & \textbf{3.82 $\pm$ {\footnotesize 0.05}}  & \textbf{6.91 $\pm$ {\footnotesize 0.11}}  & \textbf{0.192 $\pm$ {\footnotesize 0.001}} & \textbf{3.91 $\pm$ {\footnotesize 0.26}}  & \textbf{7.18 $\pm$ {\footnotesize 0.85}}  & \textbf{0.18 $\pm$ {\footnotesize 0.001}} \\ \hline
\multirow{4}{*}{\textbf{Average}}                                    
& Baseline Pre-trained                       & 19.96                     & 24.59                      & 0.42                       & 19.96                     & 24.59                      & 0.42                       \\  
& Baseline Fine-tuned                        & 17.33 & 21.82            & 0.37 & 16.28           & 20.66            & 0.34                         \\ 
& \textbf{Reptile}~\cite{nichol2018first}             & 11.63            & 15.07  & 0.260 & 8.20 & 11.31 & 0.181 \\ %\cline{2-8}
& \textbf{Meta pre-trained (Ours)}             & 18.93 & 23.76 & 0.38 & 18.93 & 23.76 & 0.38 \\ 
& \textbf{Meta fine-tuned (Ours)}             & 7.5                 & 10.22                 & 0.197                  & 7.7                 & 10.93                 & 0.165                  \\ 
& \textbf{Meta fine-tuned (Ours w/ ROI)}            & \textbf{7.12}                      & \textbf{9.88}                         & \textbf{0.172 }                          & \textbf{7.05                         } & \textbf{9.83}                           & \textbf{0.155} \\ \Xhline{2\arrayrulewidth}
\end{tabular}}
\caption{{\color{blue} [[To-do: Update the caption]] }The overall results for adaptation on WorldExpo'10~\cite{zhang2015crosscounting} test set with $K = 1$ and $K = 5$ train images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours w/ ROI''} and \textit{``Ours w/o ROI''}. We compare the results across 5 test scenes and the last two rows represent the average score for our models. The results in bold represent the overall best result. }
\label{tab:worldexpo}
\end{table*}


% K=1
%\begin{table}[]
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\textbf{Target}}               & \multirow{2}{*}{\textbf{Methods}}       & \multicolumn{3}{c|}{\textbf{5-shot (K=5)}}                                                                                           \\
 %                                              &                                         & \multicolumn{1}{c}{MAE}                                        & \multicolumn{1}{c}{MSE}                                        & \multicolumn{1}{c|}{MDE}                                         \\ \hline
%\multirow{4}{*}{Scene 1}         & Pre-trained                       & 5.55                      & 6.31                      & 0.70                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 5.45 $\pm$ 0.03           & 6.23 $\pm$ 0.03           & 0.68 $\pm$ 0.004           \\ \cline{2-5} 
 %                                & \textbf{Ours w/o ROI}             & 3.47 $\pm$ 0.01           & \textbf{4.19 $\pm$ 0.01}  & 0.50 $\pm$ 0.007           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{3.19 $\pm$ 0.03}  & 4.30 $\pm$ 0.07           & \textbf{0.38 $\pm$ 0.03}   \\ \hline
%\multirow{4}{*}{Scene 2}         & Pre-trained                       & 24.07                     & 34.29                     & 0.17                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 22.74 $\pm$ 0.47          & 32.92 $\pm$ 0.66          & 0.15 $\pm$ 0.003           \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 12.05 $\pm$ 0.74          & 16.62 $\pm$ 1.10          & 0.11 $\pm$ 0.007           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{11.17 $\pm$ 1.01} & \textbf{15.50 $\pm$ 1.18} & \textbf{0.11 $\pm$ 0.012}  \\ \hline
%\multirow{4}{*}{Scene 3}         & Pre-trained                       & 35.54                     & 40.78                     & 0.40                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 33.89 $\pm$ 0.26          & 39.33 $\pm$ 0.25          & 0.38 $\pm$ 0.03            \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 8.15 $\pm$ 0.17           & 11.04 $\pm$ 0.42          & 0.098 $\pm$ 0.04           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{8.07 $\pm$ 0.23}  & \textbf{10.92 $\pm$ 0.21} & \textbf{0.10 $\pm$ 0.007}  \\ \hline
%\multirow{4}{*}{Scene 4}         & Pre-trained                       & 23.95                     & 28.57                     & 0.19                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 15.69 $\pm$ 0.28          & 18.96 $\pm$ 0.27          & 0.14 $\pm$ 0.003           \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 16.64 $\pm$ 0.24          & 20.35 $\pm$ 0.25          & 0.14 $\pm$ 0.002           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{15.55 $\pm$ 0.09} & \textbf{18.94 $\pm$ 0.12} & \textbf{0.13 $\pm$ 0.001}  \\ \hline
%\multirow{4}{*}{Scene 5}         & Pre-trained                       & 10.70                     & 13.0                      & 0.67                       \\ \cline{2-5} 
%                                 & Fine-tuned                        & 8.9 $\pm$ 0.05            & 11.7 $\pm$ 0.04           & 0.50 $\pm$ 0.03            \\ \cline{2-5} 
%                                 & \textbf{Ours w/o ROI}             & 4.09 $\pm$ 0.01           & 7.36 $\pm$ 0.01           & 0.196 $\pm$ 0.01           \\ \cline{2-5} 
%                                 & \textbf{Ours with ROI}            & \textbf{3.82 $\pm$ 0.05}  & \textbf{6.91 $\pm$ 0.11}  & \textbf{0.192 $\pm$ 0.001} \\ \hline
%\end{tabular}
%\caption{The overall results for adaptation on WorldExpo test set with $K = 1$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours with ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result achieved by our model.}
%\label{tab:worldexpo_k1}
%\end{table}

% K = 5
%\begin{table}[]
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\textbf{Target}}               & \multirow{2}{*}{\textbf{Methods}}       & \multicolumn{3}{c|}{\textbf{5-shot (K=5)}}                                                                                           \\
%                                               &                                         & \multicolumn{1}{c}{MAE}                                        & \multicolumn{1}{c}{MSE}                                        & \multicolumn{1}{c|}{MDE}                                         \\ \hline
%\multirow{4}{*}{Scene 1}                       & Pre-trained                             & 5.55                                       & 6.31                                       & 0.70                                        \\ \cline{2-5} 
%                                               & Fine-tuned                              & 5.06 $\pm$ 0.11                            & 5.88 $\pm$ 0.10                            & 0.63 $\pm$ 0.005                            \\ \cline{2-5} 
%                                               & \textbf{Ours w/o ROI}  & 3.42 $\pm$ 0.03                            & 4.81 $\pm$ 0.007                           & \textbf{0.29 $\pm$ 0.04}   \\ \cline{2-5} 
%                                               & \textbf{Ours with ROI} & \textbf{3.05 $\pm$ 0.06}  & \textbf{4.19 $\pm$ 0.15}  & 0.31 $\pm$ 0.08                             \\ \hline
%\multirow{4}{*}{Scene 2}                       & Pre-trained                             & 24.07                                      & 34.29                                      & 0.17                                        \\ \cline{2-5} 
%                                               & Fine-tuned                              & 20.84 $\pm$ 1.03                           & 30.49 $\pm$ 1.37                           & 0.156 $\pm$ 0.001                           \\ \cline{2-5} 
%                                               & \textbf{Ours w/o ROI}  & 11.41 $\pm$ 0.54                           & 15.35 $\pm$ 0.51                           & 0.11 $\pm$ 0.015                            \\ \cline{2-5} 
%                                               & \textbf{Ours with ROI} & \textbf{10.73 $\pm$ 0.36} & \textbf{14.95 $\pm$ 0.60} & \textbf{0.10 $\pm$ 0.003}  \\ \hline
%\multirow{4}{*}{Scene 3}                       & Pre-trained                             & 35.54                                      & 40.78                                      & 0.40                                        \\ \cline{2-5} 
%                                               & Fine-tuned                              & 31.05 $\pm$ 0.41                           & 36.70 $\pm$ 0.43                           & 0.34 $\pm$ 0.004                            \\ \cline{2-5} 
%                                               & \textbf{Ours w/o ROI}  & 8.31 $\pm$ 0.54                            & \textbf{10.75 $\pm$ 0.54} & 0.109 $\pm$ 0.009                           \\ \cline{2-5} 
%                                               & \textbf{Ours with ROI} & \textbf{8.18 $\pm$ 0.24}  & 10.96 $\pm$ 0.31                           & \textbf{0.098 $\pm$ 0.002} \\ \hline
%\multicolumn{1}{|l|}{\multirow{4}{*}{Scene 4}} & Pre-trained                             & 23.95                                      & 28.57                                      & 0.19                                        \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & Fine-tuned                              & 16.67 $\pm$ 0.10                           & 19.70 $\pm$ 0.16                           & 0.15 $\pm$ 0.002                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours w/o ROI}  & 16.92 $\pm$ 0.52                           & 20.07 $\pm$ 0.49                           & 0.15 $\pm$ 0.004                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours with ROI} & \textbf{11.65 $\pm$ 0.59} & \textbf{15.26 $\pm$ 0.94} & \textbf{0.09 $\pm$ 0.05}   \\ \hline
%\multicolumn{1}{|l|}{\multirow{4}{*}{Scene 5}} & Pre-trained                             & 10.70                                      & 13.0                                       & 0.67                                        \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & Fine-tuned                              & 7.79 $\pm$ 0.35                            & 10.57 $\pm$ 0.66                           & 0.44 $\pm$ 0.015                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours w/o ROI}  & 4.28 $\pm$ 0.14                            & 7.68 $\pm$ 0.60                            & 0.20 $\pm$ 0.001                            \\ \cline{2-5} 
%\multicolumn{1}{|l|}{}                         & \textbf{Ours with ROI} & \textbf{3.91 $\pm$ 0.26}  & \textbf{7.18 $\pm$ 0.85}  & \textbf{0.187 $\pm$ 0.001} \\ \cline{1-5} 
%\end{tabular}
%\caption{The overall results for adaptation on WorldExpo test set with $K = 5$ images. We compare the two baselines \textit{pre-trained} and \textit{fine-tuned} with our models \textit{``Ours with ROI''} and \textit{``Ours w/o ROI''}. The results in bold represent the overall best result achieved by our model.}
%\label{tab:worldexpo_k5}
%\end{table}

%\begin{table}[]
%\centering
%\tiny
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\textbf{Methods}    & \textbf{Scene 1} & \textbf{Scene 2} & \textbf{Scene 3} & \textbf{Scene 4} & \textbf{Scene 5} & \textbf{Average} \\ \hline
%Chen et al.         & \textbf{2.1}     & 55.9             & 9.6              & 11.3             & 3.4              & 16.5             \\ \hline
%Zhang et al.        & 9.8              & 14.1             & 14.3             & 22.2             & 3.7              & 12.9             \\ \hline
%MCNN                & 3.4              & 20.6             & 12.9             & 13.0             & 8.1              & 11.6             \\ \hline
%Shang et al.        & 7.8              & 15.4             & 14.9             & 11.8             & 5.8              & 11.7             \\ \hline
%Switching-CNN       & 4.4              & 15.7             & 10.0             & 11.0             & 5.9              & 9.4              \\ \hline
%CP-CNN              & 2.9              & 14.7             & 10.5             & 10.4             & 5.8              & 8.86             \\ \hline
%CSRNet              & 2.9              & 11.5             & 8.6              & 16.6             & 3.4              & 8.6              \\ \hline
%SANet               & 2.6              & 13.2             & 9.0              & 13.3             & \textbf{3.0}     & 8.2              \\ \hline
%PACNN               & 2.3              & 12.5             & 9.1              & \textbf{11.2}    & 3.8              & 7.8              \\ \hline
%\textbf{Ours (K=1)} & 3.1              & 11.1             & \textbf{8.0}     & 15.5             & 3.8              & 8.3              \\ \hline
%\textbf{Ours (K=5)} & 3.0              & \textbf{10.7}    & 8.1              & 11.6             & 3.9              & \textbf{7.4}     \\ \hline
%\end{tabular}
%\caption{Comparison of our approach with previous approaches in Crowd Counting based on the average scores of WorldExpo test set. <\textbf{To-Do}: References>}
%\end{table}

